ROAD: Learning an Implicit Recursive Octree Auto-Decoder to Efficiently Encode 3D Shapes

Compact and accurate representations of 3D shapes are central to many perception and robotics tasks. State-of-the-art learning-based methods can reconstruct single objects but scale poorly to large datasets. We present a novel recursive implicit representation to efficiently and accurately encode large datasets of complex 3D shapes by recursively traversing an implicit octree in latent space. Our implicit Recursive Octree Auto-Decoder (ROAD) learns a hierarchically structured latent space enabling state-of-the-art reconstruction results at a compression ratio above 99%. We also propose an efficient curriculum learning scheme that naturally exploits the coarse-to-fine properties of the underlying octree spatial representation. We explore the scaling law relating latent space dimension, dataset size, and reconstruction accuracy, showing that increasing the latent space dimension is enough to scale to large shape datasets. Finally, we show that our learned latent space encodes a coarse-to-fine hierarchical structure yielding reusable latents across different levels of details, and we provide qualitative evidence of generalization to novel shapes outside the training set.

==> tables/extraction.tex <==
\begin{algorithm}[hbt!]
	\KwIn{ 
			$\textbf{l} \in \mathbb{L}$ grid levels,
			$\textbf{z}_{obj} \in \mathbb{R}^{N}$ latent vectors 
		}
		\KwOut{ 
			$\textbf{pcd} \in \mathbb{R}^3$ surface points,
			$\textbf{nrm} \in \mathbb{N}^3$ normals
% 			$\textbf{col} \in \mathbb{C}^3$ colors
		}
		
		\tcc{Recursively subdivide voxels until desired LoD is reached}
% 		$sum = 0$ \;
		\For{$ d \in \{1, \ldots, D\} $}{
            $\textbf{z}_{d+1}, \textbf{o}_{d+1}, \textbf{s}_{d+1}, \textbf{n}_{d+1} \leftarrow \text{ROAD}(\textbf{z}_{d})$ \tcp*{subdivide cells}
			$\textbf{z}_{d+1}, \textbf{s}_{d+1}, \textbf{n}_{d+1} \leftarrow \textbf{z}_{d+1}[\textbf{o}_{d+1}], \textbf{s}_{d+1}[\textbf{o}_{d+1}], \textbf{n}_{d+1}[\textbf{o}_{d+1}]$ \tcp*{remove unoccupied cells}
			
		}
		\tcc{Extract object shape}
		$\textbf{p} \leftarrow \textbf{x} - \textbf{n} * \textbf{s}$ \tcp*{project points onto the surface}
		\KwRet{$\textbf{p}$, $\textbf{n}$}
		
		\caption{Octree-based recursive surface extraction}
		\label{alg:octree}
	\end{algorithm}

==> tables/nglod.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{8pt}
% \resizebox{6cm}{!}{
    \begin{tabular}{c|c|c}
    \toprule
          & NGLOD~\cite{takikawa2021neural}$\dagger$ $+$ Thingi32~\cite{zhou2016thingi10k} & NGLOD~\cite{takikawa2021neural} + Ours \\
    \midrule
    IoU LoD 1 & 96.5  & 96.0 \\
    IoU LoD 2 & 97.9  & 97.4 \\
    IoU LoD 3 & 98.8  & 97.9 \\
    IoU LoD 4 & 99.2  & 98.1 \\
    IoU LoD 5 & 99.3 & 98.0 \\
    Chamfer LoD 5 & 0.0296 & \color{red}{0.0653} \\
    \bottomrule
    \end{tabular}%
    % }
     \caption{\textbf{Downstream reconstruction task using NGLOD~\cite{takikawa2021neural}.} Middle column: we train one NGLOD~\cite{takikawa2021neural} model for each shape in Thingi32~\cite{zhou2016thingi10k}; we compute the reconstruction metrics by comparing against the Thingi32 shapes. Right column: we use our method to train one model that encodes all the Thingi32 models, and we subsequently train one NGLOD model for each shape encoded by our model; we compute the reconstruction metrics by comparing against the \textit{original} Thingi32 shapes.}
    %  \color{red}{Not sure these results are helping us. They're good, but at first glance it could look like our method is worse, and it would be unclear why to someone who's not reading carefully. Also, our chamfer is way off (it should be ~0.035) due to something with model 58168.}
  \label{tab:nglod}%
\end{table} 


			
